Bridging the Gap: FPGAs as Programmable Switches

The emergence of P4, a domain specific language, coupled to PISA, a domain specific architecture, is revolutionizing the networking field. P4 allows to describe how packets are processed by a programmable data plane, spanning ASICs and CPUs, implementing PISA. Because the processing flexibility can be limited on ASICs, while the CPUs performance for networking tasks lag behind, recent works have proposed to implement PISA on FPGAs. However, little effort has been dedicated to analyze whether FPGAs are good candidates to implement PISA. In this work, we take a step back and evaluate the micro-architecture efficiency of various PISA blocks. We demonstrate, supported by a theoretical and experimental analysis, that the performance of a few PISA blocks is severely limited by the current FPGA architectures. Specifically, we show that match tables and programmable packet schedulers represent the main performance bottlenecks for FPGA-based programmable switches. Thus, we explore two avenues to alleviate these shortcomings. First, we identify network applications well tailored to current FPGAs. Second, to support a wider range of networking applications, we propose modifications to the FPGA architectures which can also be of interest out of the networking field.

==> fig_busvsfreq.tex <==
%auto-ignore
\begin{tikzpicture}
	\pgfplotsset{compat=1.4}
	\pgfplotsset{	set layers,
		scale only axis,
		width=0.3928\textwidth, height=3.6cm,
		xtick=data,xtick pos = bottom,
                ytick align=outside,
                xtick align=outside,
                tickwidth=0.075cm,
		yticklabel={\pgfmathprintnumber[assume math mode=true]{\tick}},
		yticklabel style={font=\scriptsize},
		xlabel={Bus size [bits]},
                yticklabel shift=-2pt,
                xticklabel shift=-4pt,
                xlabel shift = -7pt,
                xmin=20, xmax=2090,
		xlabel style={font=\scriptsize},
		xticklabel={\pgfmathprintnumber[assume math mode=true]{\tick}},
		xticklabel style={font=\scriptsize, rotate=45, /pgf/number format/1000 sep={}}
	}	
%	bus = [ 64, 128, 256, 512, 1024, 1280, 2048 ]
%	ff = [ 45.287, 52.707, 60.763, 80.451, 122.695, 160.261, 238.616]
%	lut = [ 28.764, 34.875, 43.856, 63.792, 109.630, 143.186, 225.563]
%	bram = [ 72, 79.5, 92, 116.5, 167, 193, 269]
%	clock = [ 1.936, 1.975, 1.965, 2.060, 2.101, 2.472, 2.604]
        \definecolor{aqua}{rgb}{0.0, 1.0, 1.0}
	\begin{axis}[
	    ymin=0,
	    ymax=290,
	    ytick distance=50,
	    axis y line*=left,
	    ylabel={FFs/LUTs ($\times$ 1000), BRAMs},
	    ylabel style={ font=\scriptsize},
            ylabel shift = -4pt,
	  ]	
	  \addplot [thick, red, mark=*, mark options={fill=red, draw=none}] 
	  coordinates {(64,45.287) (128,52.707) (256,60.763) (512,80.451) (1024,122.695) (1280,160.261) (2048,238.616)};\label{plot_FF2}
	  \addplot [thick, blue, mark=square*, mark options={fill=blue, draw=none}] 
	  coordinates {(64,28.764) (128,34.875) (256,43.856) (512,63.792) (1024,109.630) (1280,143.186) (2048,225.563)};\label{plot_LUT2}
	  \addplot [thick, aqua, mark=diamond*, mark options={fill=aqua, draw=none}] 
	  coordinates {(64,72) (128,79.5) (256,92) (512,116.5) (1024,167) (1280,193) (2048,269)};\label{plot_BRAM2}
%		\addplot[xshift=-0.5*\pgfplotbarwidth, fill=red] coordinates {(T0,241.656) (T1,513.126) (T2,523.813) (T3,538.252) (T4,698.678) (T5,520.916)}; \label{plot_FF}
%		\addplot[xshift=-0.5*\pgfplotbarwidth, fill=blue] coordinates {(T0,230.632) (T1,494.573) (T2,501.373) (T3,510.845) (T4,804.417) (T5,497.138)}; \label{plot_LUT}
%		\addplot[xshift=-0.5*\pgfplotbarwidth, fill=green] coordinates {(T0,269) (T1,495.5) (T2,495.5) (T3,694) (T4,583.5) (T5,495.5)}; \label{plot_BRAM}
	\end{axis}
	\begin{axis}[
	    axis y line*=right,
	    axis x line=none,
	    ymin=0,
	    ymax=3.0,
	    ytick distance=0.5,
	    legend cell align={left},
	    ylabel={Clock Period [ns]},
	    ylabel style={ font=\scriptsize},
	    legend style={at={(0.97,0.03)},anchor=south east,font=~\scriptsize, nodes={inner sep=0.5pt}},
            yticklabel style={
              /pgf/number format/.cd,
              fixed,
              fixed zerofill,
              precision=1,
              /tikz/.cd},
            ylabel shift = -5pt
	  ]
		\addlegendimage{/pgfplots/refstyle=plot_FF2, mark options={scale=1}}\addlegendentry{FFs}
		\addlegendimage{/pgfplots/refstyle=plot_LUT2, mark options={scale=1}}\addlegendentry{LUTs}
		\addlegendimage{/pgfplots/refstyle=plot_BRAM2, mark options={scale=1}}\addlegendentry{BRAM}	
		\addplot[mark=triangle*, only marks, mark options={fill,green!60!black, draw=none}] coordinates {(64,1.936) (128,1.975) (256,1.965) (512,2.060) (1024,2.101) (1280,2.472) (2048,2.604)};\label{plot_CP2}
		\addlegendentry{Clock Period}

	\end{axis}
\end{tikzpicture}


==> modules/circuitDesignLibrary.tex <==
%auto-ignore
%this file contains shape declaration and macro that define 
 %basic computer science shape for Hardware design.
 %this file should be include in the preamble
 
 \catcode`@=11

\pgfkeys{%
  /pgf/logicalbloc io north/.initial=5,
%  /pgf/logicalbloc io south/.initial=10,
%  /pgf/logicalbloc io east/.initial=10,
  /pgf/logicalbloc io west/.initial=10,
  /pgf/logicalbloc io north spacing/.initial=0.15cm,
%  /pgf/logicalbloc io south spacing/.initial=0.25cm,
%  /pgf/logicalbloc io east spacing/.initial=0.25cm,
  /pgf/logicalbloc io west spacing/.initial=0.20cm
}
\def\maxpins{100}


%stdChip
\pgfdeclareshape{logicalbloc}{
	\savedanchor\centerpoint{% 
		\pgf@x=.5\wd\pgfnodeparttextbox%
		\pgf@y=.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by-.5\dp\pgfnodeparttextbox%
	  }
	  \anchor{center}{\centerpoint}
	  
	  \saveddimen\height{%
		\pgfmathsetlength\pgf@x{(\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing}}%
	  }
	  \saveddimen\width{%
		\pgfmathsetlength\pgf@y{(\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing}}%
	  }
	  \saveddimen{\yspacing}{\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logicalbloc io west spacing}}}	  
	  \saveddimen{\xspacing}{\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/logicalbloc io north  spacing}}}
	  
	  \backgroundpath{%
		\pgfpathrectanglecorners{\pgfpointadd{\centerpoint}{\genbottomleftpoint}}%
		{\pgfpointadd{\centerpoint}{\gentoprightpoint}}%
	  }
 

	  \pgfmathloop%
	  \ifnum\pgfmathcounter>\maxpins\relax% 
	  \else%
		% Need to expand \pgfmathcounter
		\edef\marshal{\noexpand\anchor{io east \pgfmathcounter}}%
		\expandafter\marshal\expandafter{\expandafter\chippinanchorright\expandafter{\pgfmathcounter}}%
	  \repeatpgfmathloop%
	  
	  \pgfmathloop%
	  \ifnum\pgfmathcounter>\maxpins\relax% 
	  \else%
		% Need to expand \pgfmathcounter
		\edef\marshal{\noexpand\anchor{io north \pgfmathcounter}}%
		\expandafter\marshal\expandafter{\expandafter\chippinanchorupper\expandafter{\pgfmathcounter}}%
	  \repeatpgfmathloop%
	  
	  \pgfmathloop%
	  \ifnum\pgfmathcounter>\maxpins\relax% 
	  \else%
		% Need to expand \pgfmathcounter
		\edef\marshal{\noexpand\anchor{io south \pgfmathcounter}}%
		\expandafter\marshal\expandafter{\expandafter\chippinanchorbottom\expandafter{\pgfmathcounter}}%
	  \repeatpgfmathloop%
	  
	  \pgfmathloop%
	  \ifnum\pgfmathcounter>\maxpins\relax% 
	  \else%
		% Need to expand \pgfmathcounter
		\edef\marshal{\noexpand\anchor{io west \pgfmathcounter}}%
		\expandafter\marshal\expandafter{\expandafter\chippinanchorleft\expandafter{\pgfmathcounter}}%
	  \repeatpgfmathloop%
}

\def\genbottomleftpoint{%
%	\pgfmathsetlength{pgf@xb}{(\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing}}%
%	\pgfmathsetlength{pgf@yb}{(\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing}}%
%	\setlength{\pgf@xa}{1cm}
%	\setlength{\pgf@ya}{1cm}
%	\if \pgf@xb<\pgf@xa
%		\if \pgf@yb<\pgf@ya
%			\pgfpoint{-0.5cm}{-0.5cm}
%		\else
%			\pgfpoint{-0.5cm}{-(\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing}/2}
%		\fi
%	\else
%		\if \pgf@yb<\pgf@ya
%			\pgfpoint{-(\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing}/2}{-0.5cm}
%		\else
			\pgfpoint{-((\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing})/2}{-((\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing})/2}
%		\fi
%	\fi
}
\def\gentoprightpoint{%
%	\if {\pgfkeysvalueof{/pgf/logicalbloc io west} < \pgfkeysvalueof{/pgf/logicalbloc io east}}
%		\setlength{\pgf@xc}{1cm}
%	\else
%		\setlength{\pgf@xc}{1cm}
%	\fi
%	\if
%		\setlength{\pgf@xc}{1cm}
%	\else
%		\setlength{\pgf@xc}{1cm}
%	\fi
%	\pgfmathsetlength{pgf@xb}{(\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing}}%
%	\pgfmathsetlength{pgf@yb}{(\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing}}%
%	\setlength{\pgf@xa}{1cm}
%	\setlength{\pgf@ya}{1cm}
%	\if \pgf@xb<\pgf@xa
%		\if \pgf@yb<\pgf@ya
%			\pgfpoint{0.5cm}{0.5cm}
%		\else
%			\pgfpoint{0.5cm}{(\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing}/2}
%		\fi
%	\else
%		\if \pgf@yb<\pgf@ya
%			\pgfpoint{(\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing}/2}{0.5cm}
%		\else
			\pgfpoint{((\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing})/2}{((\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing})/2}
%		\fi
%	\fi
}


\def\genpointbottom#1{
\pgfpoint{(\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing}/2-#1*\xspacing}{-(\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing}/2}
}

\def\chippinanchorbottom#1{%
	  % When this macro is called,
	  % \centerpoint, \height and \chipspacing will be defined.
	  %\pgfpointadd{\centerpoint}{\pgfpoint{\width/2-#1*\xspacing}{-\height/2}}%
	  \pgfpointadd{\centerpoint}{\genpointbottom{#1}}%
}

\def\genpointupper#1{
\pgfpoint{(\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing}/2-#1*\xspacing}{(\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing}/2}
}

\def\chippinanchorupper#1{%
	  % When this macro is called,
	  % \centerpoint, \height and \chipspacing will be defined.
	  \pgfpointadd{\centerpoint}{\genpointupper{#1}}%
}

\def\genpointleft#1{
\pgfpoint{-(\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing}/2}{(\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing}/2-#1*\yspacing}
}

\def\chippinanchorleft#1{%
	  % When this macro is called,
	  % \centerpoint, \height and \chipspacing will be defined.
	  \pgfpointadd{\centerpoint}{\genpointleft{#1}}%
}

\def\genpointright#1{
\pgfpoint{(\pgfkeysvalueof{/pgf/logicalbloc io north}+1)*\pgfkeysvalueof{/pgf/logicalbloc io north spacing}/2}{(\pgfkeysvalueof{/pgf/logicalbloc io west}+1)*\pgfkeysvalueof{/pgf/logicalbloc io west spacing}/2-#1*\yspacing}
}
\def\chippinanchorright#1{%
	  % When this macro is called,
	  % \centerpoint, \height and \chipspacing will be defined.
	  \pgfpointadd{\centerpoint}{\genpointright{#1}}%
}

\catcode`@=12


==> modules/grammarSpec.tex <==
%auto-ignore
\newlength\grammarLongest
\newlength\grammarLeftMargin
\makeatletter
\newenvironment{grammarC}[1]{%
\list{}{%
\settowidth\grammarLongest{#1}
\setlength\grammarLeftMargin{\dimexpr0.5\linewidth-0.5\grammarLongest}
\labelwidth\grammarindent%
\leftmargin\dimexpr\grammarindent+\grammarLeftMargin\relax%
\advance\grammarindent\labelsep
\itemindent\z@%
\listparindent\z@%
\parsep\grammarparsep%
}%
\let\\\@normalcr
\syntaxShortcuts\relax\relax%
\def\alt{\\\llap{\textbar\quad}}%
\def\gr@setpar{%
\def\par{%
\parshape\@ne\@totalleftmargin\linewidth%
\@@par%
\catcode`\<12%
\everypar{%
\everypar{}%
\catcode`\<\active%
\gr@implitem%
}%
}%
}%
\gr@setpar%
\par%
\let\gr@leftsq\[%
\let\gr@rightsq\]%
\def\gr@endsyntdiag]{\end{syntdiag}\gr@setpar\par}%
\def\[{\@ifnextchar[{\begin{syntdiag}\@gobble}\gr@leftsq}%
\def\]{\@ifnextchar]\gr@endsyntdiag\gr@rightsq}%
}{%
\@newlistfalse%
\everypar{}%
\endlist%
}
\makeatother


==> myTikzShape.tex <==
%auto-ignore

\makeatletter
%%only width is taken into consideration height=0.3width 
\pgfdeclareshape{cryptKeyPrivate}{
	% The 'minimum width' and 'minimum height' keys, not the content, determine
	% the size
	\savedanchor\northeast{%
		\pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
		\pgfmathsetlength\pgf@y{0.5*\pgfshapeminwidth/(1+(1+cos(30))*0.2)}%
		\pgf@x=0.5\pgf@x
		\pgf@y=0.5\pgf@y
	}
	
	% This is redundant, but makes some things easier:
	\savedanchor\southwest{%
		\pgfmathsetlength\pgf@x{1*\pgfshapeminwidth}%
		\pgfmathsetlength\pgf@y{0.5*\pgfshapeminwidth/(1+(1+cos(30))*0.2)}%
		\pgf@x=-0.5\pgf@x
		\pgf@y=-0.5\pgf@y
	}
	% Inherit from rectangle
	\inheritanchorborder[from=rectangle]
	
	% Define same anchor a normal rectangle has
	\anchor{center}{\pgfpointorigin}
	\anchor{north}{\northeast \pgf@x=0pt}
	\anchor{east}{\northeast \pgf@y=0pt}
	\anchor{south}{\southwest \pgf@x=0pt}
	\anchor{west}{\southwest \pgf@y=0pt}
	\anchor{north east}{\northeast}
	\anchor{north west}{\northeast \pgf@x=-\pgf@x}
	\anchor{south west}{\southwest}
	\anchor{south east}{\southwest \pgf@x=-\pgf@x}
	\anchor{text}{
		\pgfpointorigin
		\advance\pgf@x by -.5\wd\pgfnodeparttextbox%
		\advance\pgf@y by -.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by +.5\dp\pgfnodeparttextbox%
	}
	
	
	% Draw the rectangle box and the port labels
	\backgroundpath{
		\pgfmathsetlength\pgf@xa{\pgfshapeminwidth/(1+(1+cos(30))*0.2)}
		\southwest
		\pgfmathsetlength\pgf@xb{(1+cos(30))*0.2*\pgf@xa}
		\advance\pgf@x by \pgf@xb
		\pgf@xb=\pgf@x \pgf@yb=\pgf@y
		\pgf@xc=\pgf@x \pgf@yc=\pgf@y
		
		%point a
		\pgfmathsetlength\pgf@y{0.4*\pgf@xa}
		\advance\pgf@yb by \pgf@y
		
		%point b
		\pgfmathsetlength\pgf@x{\pgf@xa}
		\pgfmathsetlength\pgf@y{0.2*\pgf@xa}
		\advance\pgf@xc by \pgf@x
		\advance\pgf@yc by \pgf@y
		
		\pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
		
		%point c
		\pgfmathsetlength\pgf@x{0.9*\pgf@xa}
		\pgfmathsetlength\pgf@y{-0.3*\pgf@xa}
		\advance\pgf@xb by \pgf@x
		\advance\pgf@yb by \pgf@y
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		
		%point d
		\pgfmathsetlength\pgf@x{-0.2*\pgf@xa}
		\pgfmathsetlength\pgf@y{-0.2*\pgf@xa}
		\advance\pgf@xc by \pgf@x
		\advance\pgf@yc by \pgf@y
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
		
		%point e
		\pgfmathsetlength\pgf@x{-0.2*\pgf@xa}
		\pgfmathsetlength\pgf@y{0*\pgf@xa}
		\advance\pgf@xb by \pgf@x
		\advance\pgf@yb by \pgf@y
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		
		%point f
		\pgfmathsetlength\pgf@x{-0.2*\pgf@xa}
		\pgfmathsetlength\pgf@y{0.2*\pgf@xa}
		\advance\pgf@xc by \pgf@x
		\advance\pgf@yc by \pgf@y
		
		
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
		
		
		\pgfmathsetlength\pgf@x{-0.7*\pgf@xa}		
		\advance\pgf@xb by \pgf@x
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
		
		\pgfmathsetlength\pgf@xb{0.2*\pgf@xa}	
		\pgfpatharc{-30}{-330}{\pgf@xb}
		
		\pgfclosepath	
		\southwest
		\pgf@xc=\pgf@x \pgf@yc=\pgf@y
		\pgfmathsetlength\pgf@xb{0.05*\pgf@xa}	
		\pgfmathsetlength\pgf@x{0.1*\pgf@xa}	
		\pgfmathsetlength\pgf@y{0.3*\pgf@xa}		
		\advance\pgf@xc by \pgf@x
		\advance\pgf@yc by \pgf@y
		\pgfpathcircle{\pgfpoint{\pgf@xc}{\pgf@yc}}{\pgf@xb} %(-2.4,-1)
	}
}

\pgfdeclareshape{cryptKeyPublic}{
	% The 'minimum width' and 'minimum height' keys, not the content, determine
	% the size
	\savedanchor\northeast{%
		\pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
		\pgfmathsetlength\pgf@y{0.5*\pgfshapeminwidth/(1+(1+cos(30))*0.2)}%
		\pgf@x=0.5\pgf@x
		\pgf@y=0.5\pgf@y
	}

	% This is redundant, but makes some things easier:
	\savedanchor\southwest{%
		\pgfmathsetlength\pgf@x{1*\pgfshapeminwidth}%
		\pgfmathsetlength\pgf@y{0.5*\pgfshapeminwidth/(1+(1+cos(30))*0.2)}%
		\pgf@x=-0.5\pgf@x
		\pgf@y=-0.5\pgf@y
	}
	% Inherit from rectangle
	\inheritanchorborder[from=rectangle]
	
	% Define same anchor a normal rectangle has
	\anchor{center}{\pgfpointorigin}
	\anchor{north}{\northeast \pgf@x=0pt}
	\anchor{east}{\northeast \pgf@y=0pt}
	\anchor{south}{\southwest \pgf@x=0pt}
	\anchor{west}{\southwest \pgf@y=0pt}
	\anchor{north east}{\northeast}
	\anchor{north west}{\northeast \pgf@x=-\pgf@x}
	\anchor{south west}{\southwest}
	\anchor{south east}{\southwest \pgf@x=-\pgf@x}
	\anchor{text}{
		\pgfpointorigin
		\advance\pgf@x by -.5\wd\pgfnodeparttextbox%
		\advance\pgf@y by -.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by +.5\dp\pgfnodeparttextbox%
	}
	
	
	% Draw the rectangle box and the port labels
	\backgroundpath{
		\pgfmathsetlength\pgf@xa{\pgfshapeminwidth/(1+(1+cos(30))*0.2)}
		\southwest
		\pgfmathsetlength\pgf@xb{(1+cos(30))*0.2*\pgf@xa}
		\advance\pgf@x by \pgf@xb
		\pgf@xb=\pgf@x \pgf@yb=\pgf@y
		\pgf@xc=\pgf@x \pgf@yc=\pgf@y
		
		%point a
		\pgfmathsetlength\pgf@y{0.4*\pgf@xa}
		\advance\pgf@yb by \pgf@y
		
		%point b
		\pgfmathsetlength\pgf@x{\pgf@xa}
		\pgfmathsetlength\pgf@y{0.2*\pgf@xa}
		\advance\pgf@xc by \pgf@x
		\advance\pgf@yc by \pgf@y
		
		\pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
		
		%point c
		\pgfmathsetlength\pgf@x{0.9*\pgf@xa}
		\pgfmathsetlength\pgf@y{-0.4*\pgf@xa}
		\advance\pgf@xb by \pgf@x
		\advance\pgf@yb by \pgf@y
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		
		%point d
		\pgfmathsetlength\pgf@x{-0.2*\pgf@xa}
		\pgfmathsetlength\pgf@y{-0.1*\pgf@xa}
		\advance\pgf@xc by \pgf@x
		\advance\pgf@yc by \pgf@y
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
		
		%point e
		\pgfmathsetlength\pgf@x{-0.2*\pgf@xa}
		\pgfmathsetlength\pgf@y{0*\pgf@xa}
		\advance\pgf@xb by \pgf@x
		\advance\pgf@yb by \pgf@y
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}

		%point f
		\pgfmathsetlength\pgf@x{-0.2*\pgf@xa}
		\pgfmathsetlength\pgf@y{0.1*\pgf@xa}
		\advance\pgf@xc by \pgf@x
		\advance\pgf@yc by \pgf@y

		
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
		
				
		\pgfmathsetlength\pgf@x{-0.7*\pgf@xa}		
		\advance\pgf@xb by \pgf@x
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
		
		\pgfmathsetlength\pgf@xb{0.2*\pgf@xa}	
		\pgfpatharc{-30}{-330}{\pgf@xb}

		\pgfclosepath	
		\southwest
		\pgf@xc=\pgf@x \pgf@yc=\pgf@y
		\pgfmathsetlength\pgf@xb{0.05*\pgf@xa}	
		\pgfmathsetlength\pgf@x{0.1*\pgf@xa}	
		\pgfmathsetlength\pgf@y{0.3*\pgf@xa}		
		\advance\pgf@xc by \pgf@x
		\advance\pgf@yc by \pgf@y
		\pgfpathcircle{\pgfpoint{\pgf@xc}{\pgf@yc}}{\pgf@xb} %(-2.4,-1)

	}
}

\makeatother

